When to Accept Automated Predictions and When to Defer to Human Judgment?

Ensuring the reliability and safety of automated decision-making is crucial. It is well-known that data distribution shifts in machine learning can produce unreliable outcomes. This paper proposes a new approach for measuring the reliability of predictions under distribution shifts. We analyze how the outputs of a trained neural network change using clustering to measure distances between outputs and class centroids. We propose this distance as a metric to evaluate the confidence of predictions under distribution shifts. We assign each prediction to a cluster with centroid representing the mean softmax output for all correct predictions of a given class. We then define a safety threshold for a class as the smallest distance from an incorrect prediction to the given class centroid. We evaluate the approach on the MNIST and CIFAR-10 datasets using a Convolutional Neural Network and a Vision Transformer, respectively. The results show that our approach is consistent across these data sets and network models, and indicate that the proposed metric can offer an efficient way of determining when automated predictions are acceptable and when they should be deferred to human operators given a distribution shift.

==> Archive/05-Results-total.tex <==
%%%%%%%%%%%
% RESULTS %
%%%%%%%%%%%

% \section{Results - Total}

% Moved to supplementary material
% We train our neural network, and make a record of the class probability outputs, true class and predicted class. Figure \ref{fig:mnist_combined_confusion_matrix}


% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.99\columnwidth]{Figures/mnist_combined_confusion_matrix.png}
%     \caption{Please zoom in for detail. Confusion matrices for the MNIST classification model on the training dataset (left) and testing dataset (right). The matrices display the true labels on the vertical axis and the predicted labels on the horizontal axis. The diagonal elements represent correctly classified instances, while the off-diagonal elements indicate misclassifications.}
%     \label{fig:mnist_combined_confusion_matrix}
% \end{figure}

% The accuracy on the training dataset in 98.38\% and 98.46\% on the testing dataset. Figure \ref{fig:mnist_combined_misclassifications}. We note that for both datasets, number zero is the digit less likely, and number eight is the digit most likely to be misclassified. Other digits that are less likely to be misclassified are digits one and; six in the training dataset, and five in the testing dataset. The confusion matrices in Figure \ref{fig:mnist_combined_confusion_matrix} provide some insights into what are the most likely misclassifications, for example digit eight is likely to be misclassified as six or nine, while digit three is likely to be misclassified as two, five or nine.
% For confusion matrices
% [1] Stehman, S. V. (1997). Selecting and interpreting measures of thematic classification accuracy. Remote Sensing of Environment, 62(1), 77-89.

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.99\columnwidth]{Figures/mnist_combined_misclassifications.png}
%     \caption{Normalised misclassifications for each class in the training data (left) and testing data (right). The x-axis represents the class labels from 0 to 9, with the corresponding non-normalised misclassification count displayed below each label. The y-axis shows the normalized misclassifications, obtained by dividing the misclassification count for each class by the total number of misclassifications in the respective dataset. }
%     \label{fig:mnist_combined_misclassifications}
% \end{figure}

% MOved to Context
% %%%%%%%%%%%%%%
% % CLUSTERING %
% %%%%%%%%%%%%%%

% \subsection{Clustering}

% Clustering algorithms play a crucial role in various domains, enabling the discovery of intrinsic structures and patterns within datasets. These algorithms aim to partition data points into groups or clusters based on their similarity, such that points within the same cluster are more similar to each other than to those in other clusters \citep{jain2010data}. Clustering techniques find applications in a wide range of fields, including image segmentation, anomaly detection, customer segmentation, and bioinformatics \citep{xu2015comprehensive}.

% One of the most widely used clustering algorithms is k-means, which iteratively assigns data points to the nearest cluster centroid and updates the centroids based on the assigned points \citep{lloyd1982least}. K-means is computationally efficient and scales well to large datasets, making it suitable for many practical applications. However, it requires specifying the number of clusters in advance and is sensitive to the initial placement of centroids \citep{arthur2007k}.

% Another popular clustering approach is hierarchical clustering, which builds a tree-like structure of clusters by either merging smaller clusters into larger ones (agglomerative) or dividing larger clusters into smaller ones (divisive) \citep{johnson1967hierarchical}. Hierarchical clustering provides a visual representation of the clustering process and allows for the exploration of clusters at different granularities. However, it can be computationally expensive and may not scale well to large datasets \citep{mullner2011modern}.

% Density-based clustering algorithms, such as DBSCAN (Density-Based Spatial Clustering of Applications with Noise), identify clusters as dense regions separated by areas of lower density \citep{ester1996density}. DBSCAN is particularly useful for detecting clusters of arbitrary shape and handling noise or outliers in the data. It does not require specifying the number of clusters and can discover clusters of varying densities \citep{schubert2017dbscan}.

% Clustering algorithms have found numerous applications across various domains. In image segmentation, clustering techniques are used to group pixels with similar characteristics, enabling object detection and recognition \citep{shi2000normalized}. Anomaly detection systems employ clustering to identify unusual patterns or outliers that deviate from the norm, aiding in fraud detection and network intrusion detection \citep{chandola2009anomaly}. Customer segmentation utilizes clustering to group customers with similar behaviors or preferences, facilitating targeted marketing and personalized recommendations \citep{ngai2009application}.

% In bioinformatics, clustering algorithms are extensively used for gene expression analysis, protein function prediction, and disease subtype identification \citep{eisen1998cluster}. By grouping genes or proteins with similar expression patterns or functional properties, researchers can gain insights into biological processes and discover potential biomarkers or therapeutic targets \citep{jiang2004cluster}.

% The choice of clustering algorithm depends on the specific characteristics of the data, the desired properties of the clusters, and the computational resources available. Researchers continue to develop and improve clustering techniques to address the challenges posed by high-dimensional, large-scale, and complex datasets \citep{rodriguez2019clustering}.

% In conclusion, clustering algorithms are essential tools for discovering structures and patterns in data, with applications spanning various domains. From image segmentation and anomaly detection to customer segmentation and bioinformatics, clustering techniques enable researchers and practitioners to extract valuable insights and make data-driven decisions.

% MOVED TO METHODS
% To initialise the centroids for K-Means clustering with 10 clusters, where each cluster represents a digit from the MNIST dataset, we leverage the information from the probability distribution of the correct predictions.

% The resulting centroids array will have shape (10, 10), where each row represents a centroid for a specific digit. The values in each row correspond to the average probability distribution of the correct predictions for that digit.

% To find the centroids, we use:

% \begin{algorithm}
% \caption{K-Means Centroid Initialisation for MNIST Dataset}
% \begin{algorithmic}[1]
% \Require{$correct\_preds$: array of shape $(n, 12)$, where $n$ is the number of correct predictions}
% \Ensure{$centroids$: array of shape $(10, 10)$, initialised centroids for each digit class}

% \State $probs\_dist \gets corrects\_preds[:, :10]$ \Comment{Extract probability distribution for each digit}
% \State $centroids \gets \text{zeros}((10, 10))$ \Comment{Initialise centroids array}

% \For{$digit \gets 0$ to $9$}
% \State $indices \gets \text{where}(\text{argmax}(probs\_dist, \text{axis}=1) == digit)[0]$ \Comment{Find indices of rows where digit has highest probability}
% \State $centroid \gets \text{mean}(probs\_dist[indices], \text{axis}=0)$ \Comment{Compute mean probability distribution for selected rows}
% \State $centroids[digit] \gets centroid$ \Comment{Assign centroid to corresponding row in centroids array}
% \EndFor

% \State \textbf{return} $centroids$
% \end{algorithmic}
% \end{algorithm}

% The algorithm starts with the Require statement, specifying the input correct\_preds array of shape $(n, 12)$, where $n$ is the number of correct predictions.
% The Ensure statement specifies the output centroids array of shape $(10, 10)$, which will store the initialised centroids for each digit.
% In line 1, we extract the probability distribution for each digit by selecting the first 10 columns of correct\_preds and store it in the prob\_dist array, where column 11 is the label and column 12 is the prediction, and both are the same for correct predictions.
% In line 2, we initialise the centroids array with zeros of shape $(10, 10)$ to store the centroid for each digit.
% We start a loop that iterates over each digit from 0 to 9.
% In line 4, for each digit, we find the indices of rows in prob\_dist where the digit has the highest probability using \text{argmax}(prob\_dist, \text{axis}=1) == digit. This gives us the indices of rows that are most likely to represent the current digit, which is indeed the case since all predictions are correct.
% In line 5, we compute the mean probability distribution for the selected rows using \text{mean}(prob\_dist[indices], \text{axis}=0). This gives us the centroid for the current digit.
% In line 6, we assign the computed centroid to the corresponding row in the centroids array.
% After the loop ends, we return the centroids array.

% The resulting centroids array will have shape $(10, 10)$, where each row represents a centroid for a specific digit. The values in each row correspond to the average probability distribution of the correct predictions for that digit.

% By initialising the centroids based on the probability distribution of correct predictions, we provide a good starting point for the K-Means algorithm. Each centroid will be initialised to represent the typical probability distribution for a specific digit class prediction, which helps the algorithm converge faster.

% Our k-means cluster for 59074 correct MNIST digit predictions converges in a fraction of a second. We then plot the mean distance to centroids for every class in Figure \ref{fig:MNIST_Correct_Training_and_Testing_Mean_Distance_To_Centroids}.

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.99\columnwidth]{Figures/MNIST_Correct_Training_and_Testing_Mean_Distance_To_Centroids.png}
%     \caption{Mean distances for Softmax function output for each class, for correct classifications. On the right is the plot for the training dataset and the corresponding test dataset on the right.}
%     \label{fig:MNIST_Correct_Training_and_Testing_Mean_Distance_To_Centroids}
% \end{figure}

% The plots in Figure \ref{fig:boxplots_side_by_side_x2} compare the distribution of distances to centroids for correctly and incorrectly classified instances across different digit classes in both the training and testing MNIST datasets.

% In the training data (left plot), the distances for correctly classified instances are lower than those of incorrectly classified instances across all digit classes. This indicates that the distance of the Softmax output to the K-Means cluster centroids are good candidate proxies for accuracy, leading to smaller distances for correct classifications.

% % Figure generated by function call:
% % boxplots_side_by_side_x2(d2c_train_correct, d2c_train_incorrect, d2c_test_correct_train_centroids, d2c_test_incorrect_train_centroids, False, True, title1="Training Data Boxplots of Softmax Distances to Training Centroids", title2="Testing Data Boxplots of Softmax Distances to Training Centroids")
% \begin{figure*}[h]
%     \centering
%     \includegraphics[width=0.99\textwidth]{Figures/boxplots_side_by_side_x2_training_centroids.png}   \captionsetup{justification=raggedright,singlelinecheck=false}
%     \caption{Distribution of Distances to Centroids for Correctly and Incorrectly Classified Instances in Training and Testing MNIST Data, where training data is on the left and testing data is displayed on the right. Distances are shown on a logarithmic scale. Note, centroids are for the correctly classified training examples, for both training and testing dataset.}
%     \label{fig:boxplots_side_by_side_x2_training_centroids}
% \end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% CIFAR10 MNIST SOFTMAX DISTANCE TO %
% CLUSTER CENTROID STATISTICS       %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{table*}[h]
% \centering
% \begin{tabular}{c|cccccc|cccccc}
% \hline
% & \multicolumn{6}{c|}{Training Dataset Correct Predictions} & \multicolumn{6}{c}{Training Dataset Incorrect Predictions} \\
% Digit & Mean & Median & Min & Max & $\sigma$ & Count & Mean & Median & Min & Max & $\sigma$ & Count \\ \hline
% 0 & 0.0166 & 0.0088 & 0.0018 & \textbf{0.8433} & 0.0536 & 5890 & 0.9955 & 0.9552 & \textbf{0.7037} & 1.3681 & 0.1756 & 33 \\
% 1 & 0.0154 & 0.0085 & 0.0020 & \textbf{0.7051} & 0.0486 & 6704 & 1.0912 & 1.0771 & \textbf{0.7247} & 1.3909 & 0.2197 & 38 \\
% 2 & 0.0370 & 0.0208 & 0.0056 & \textbf{0.7453} & 0.0746 & 5859 & 1.0409 & 1.0460 & \textbf{0.6962} & 1.3912 & 0.2064 & 99 \\
% 3 & 0.0352 & 0.0192 & 0.0055 & \textbf{0.7509} & 0.0754 & 6019 & 1.0522 & 1.0338 & \textbf{0.7139} & 1.3999 & 0.2143 & 112 \\
% 4 & 0.0295 & 0.0166 & 0.0031 & \textbf{0.6933} & 0.0661 & 5755 & 1.0681 & 1.0642 & \textbf{0.7139} & 1.4010 & 0.2045 & 87 \\
% 5 & 0.0298 & 0.0165 & 0.0024 & \textbf{0.7634} & 0.0693 & 5339 & 1.0572 & 1.0560 & \textbf{0.7066} & 1.3956 & 0.2000 & 82 \\
% 6 & 0.0154 & 0.0081 & 0.0015 & \textbf{0.7981} & 0.0485 & 5884 & 1.0485 & 1.0702 & \textbf{0.7068} & 1.4015 & 0.2110 & 34 \\
% 7 & 0.0302 & 0.0171 & 0.0028 & \textbf{0.7365} & 0.0678 & 6199 & 1.0133 & 0.9764 & \textbf{0.6960} & 1.3989 & 0.2160 & 66 \\
% 8 & 0.0619 & 0.0363 & 0.0092 & \textbf{0.7788} & 0.0989 & 5581 & 1.0232 & 1.0083 & \textbf{0.6852} & 1.3816 & 0.1990 & 270 \\
% 9 & 0.0399 & 0.0232 & 0.0048 & \textbf{0.7616} & 0.0781 & 5844 & 1.0576 & 1.0830 & \textbf{0.7179} & 1.3974 & 0.2201 & 105 \\ \hline
% & \multicolumn{6}{c|}{Testing Dataset Correct Predictions} & \multicolumn{6}{c}{Testing Dataset Incorrect Predictions} \\
% Digit & Mean & Median & Min & Max & $\sigma$ & Count & Mean & Median & Min & Max & $\sigma$ & Count \\ \hline
% 0 & 0.0141 & 0.0075 & 0.0021 & \textbf{0.7225} & 0.0506 & 977 & 1.0329 & 1.0185 & \textbf{0.7923} & 1.2880 & 0.2026 & 3 \\
% 1 & 0.0126 & 0.0071 & 0.0023 & \textbf{0.6737} & 0.0445 & 1129 & 0.9823 & 0.9556 & \textbf{0.7278} & 1.2445 & 0.1898 & 6 \\
% 2 & 0.0354 & 0.0202 & 0.0037 & \textbf{0.6697} & 0.0704 & 1015 & 1.0855 & 1.0725 & \textbf{0.7010} & 1.3833 & 0.1844 & 17 \\
% 3 & 0.0331 & 0.0177 & 0.0049 & \textbf{0.7515} & 0.0765 & 998 & 0.9823 & 0.9752 & \textbf{0.7102} & 1.3230 & 0.2044 & 12 \\
% 4 & 0.0306 & 0.0169 & 0.0047 & \textbf{0.6603} & 0.0678 & 972 & 0.9309 & 0.8725 & \textbf{0.7073} & 1.3110 & 0.1923 & 10 \\
% 5 & 0.0313 & 0.0173 & 0.0051 & \textbf{0.6324} & 0.0692 & 883 & 1.1874 & 1.2976 & \textbf{0.8477} & 1.3982 & 0.2067 & 9 \\
% 6 & 0.0172 & 0.0088 & 0.0029 & \textbf{0.7135} & 0.0545 & 941 & 1.0737 & 1.0242 & \textbf{0.7240} & 1.4009 & 0.2120 & 17 \\
% 7 & 0.0295 & 0.0165 & 0.0036 & \textbf{0.6939} & 0.0678 & 1009 & 0.9665 & 0.8833 & \textbf{0.7148} & 1.3628 & 0.2016 & 19 \\
% 8 & 0.0616 & 0.0372 & 0.0114 & \textbf{0.7328} & 0.0918 & 934 & 1.0513 & 1.0399 & \textbf{0.7252} & 1.3842 & 0.2022 & 40 \\
% 9 & 0.0359 & 0.0206 & 0.0042 & \textbf{0.6870} & 0.0765 & 980 & 1.0502 & 1.0486 & \textbf{0.6968} & 1.3838 & 0.2197 & 29 \\ \hline
% \end{tabular}
% \captionsetup{justification=raggedright,singlelinecheck=false}
% \caption{Statistical Summary of MNIST Softmax Output Distances to Centroids for Different Datasets and Prediction Outcomes. The centroids are obtained with Softmax outputs for correct class predictions from the training and testing datasets.}
% \label{tab:distance_to_centroid}
% \end{table*}

% DATA for table above
%        Mean    Median       Min       Max  Standard Deviation  Count
% 0  0.016608  0.008843  0.001769  0.843304            0.053614   5890
% 1  0.015435  0.008516  0.002036  0.705149            0.048557   6704
% 2  0.036996  0.020828  0.005605  0.745250            0.074615   5859
% 3  0.035151  0.019205  0.005478  0.750860            0.075377   6019
% 4  0.029493  0.016613  0.003111  0.693346            0.066094   5755
% 5  0.029819  0.016509  0.002448  0.763396            0.069287   5339
% 6  0.015405  0.008078  0.001526  0.798075            0.048491   5884
% 7  0.030247  0.017138  0.002791  0.736508            0.067780   6199
% 8  0.061884  0.036283  0.009184  0.778795            0.098932   5581
% 9  0.039943  0.023188  0.004768  0.761636            0.078053   5844
%        Mean    Median       Min       Max  Standard Deviation  Count
% 0  0.995516  0.955230  0.703653  1.368133            0.175639     33
% 1  1.091157  1.077065  0.724706  1.390934            0.219724     38
% 2  1.040888  1.046023  0.696177  1.391211            0.206378     99
% 3  1.052159  1.033801  0.713948  1.399858            0.214313    112
% 4  1.068138  1.064157  0.713896  1.400997            0.204490     87
% 5  1.057245  1.055964  0.706555  1.395563            0.200003     82
% 6  1.048483  1.070162  0.706828  1.401450            0.211018     34
% 7  1.013332  0.976427  0.695997  1.398902            0.216013     66
% 8  1.023217  1.008262  0.685179  1.381630            0.199017    270
% 9  1.057626  1.082991  0.717850  1.397425            0.220102    105
%        Mean    Median       Min       Max  Standard Deviation  Count
% 0  0.014064  0.007518  0.002131  0.722502            0.050551    977
% 1  0.012627  0.007062  0.002254  0.673694            0.044504   1129
% 2  0.035369  0.020174  0.003719  0.669724            0.070428   1015
% 3  0.033119  0.017744  0.004876  0.751473            0.076455    998
% 4  0.030573  0.016858  0.004709  0.660308            0.067756    972
% 5  0.031271  0.017275  0.005053  0.632375            0.069207    883
% 6  0.017175  0.008774  0.002851  0.713528            0.054455    941
% 7  0.029476  0.016466  0.003639  0.693906            0.067756   1009
% 8  0.061609  0.037214  0.011389  0.732832            0.091848    934
% 9  0.035850  0.020602  0.004236  0.686980            0.076507    980
%        Mean    Median       Min       Max  Standard Deviation  Count
% 0  1.032918  1.018475  0.792297  1.287982            0.202620      3
% 1  0.982310  0.955644  0.727825  1.244521            0.189784      6
% 2  1.085502  1.072510  0.700976  1.383269            0.184444     17
% 3  0.982309  0.975231  0.710249  1.322951            0.204446     12
% 4  0.930852  0.872484  0.707302  1.310962            0.192325     10
% 5  1.187412  1.297633  0.847685  1.398223            0.206653      9
% 6  1.073695  1.024168  0.724028  1.400876            0.211957     17
% 7  0.966459  0.883283  0.714793  1.362762            0.201621     19
% 8  1.051282  1.039866  0.725232  1.384221            0.202232     40
% 9  1.050175  1.048609  0.696760  1.383811            0.219746     29

% Figure \ref{fig:MNIST_Classification_Train_Test_Accuracy_Mean_Distance_to_Centroid_Linear_Fit} shows the linear fit for Accuracy and Mean Class Distances to Centroids.

% In the context of the MNIST dataset, the derived linear functions from the training and testing data exhibit a negative correlation between the classification accuracy and the mean class distances to the centroids. Specifically, the training data is described by the function $ y = -0.806x + 1.009 $, and the testing data by $ y = -0.677x + 1.004 $. The negative coefficients of the linear terms $ -0.806 $ and $ -0.677 $, respectively) indicate that an increase in the mean distance to the centroid correlates with a decrease in classification accuracy for both datasets.

% These results suggest a clear inverse relationship: as the mean distance from the data points in a class to their centroid increases, the propensity for correct classification diminishes. This could be due to the spread of data points within a class – greater distances from the centroid reflect a larger variance within the class, potentially making it more challenging for the classifier to identify the defining characteristics of each class accurately.

% The steeper slope for the training data function implies that accuracy is more sensitive to changes in mean distance to centroid during training. Conversely, the testing data's function has a less steep slope, which could suggest that the classifier is slightly more robust to variation in the testing set, or that the testing set has inherently less variation in mean distances across classes.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% FIGURE MNIST TRAIN TEST ACCURACY %
% VS MEAN DISTANCE TO CENTROID     %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.95\columnwidth]{Figures/MNIST_Classification_Train_Test_Accuracy_Mean_Distance_to_Centroid_Linear_Fit.png}
%     \caption{Scatter plot depicting the relationship between classification accuracy and mean class distance to the centroid for the MNIST dataset. Training data (blue dots) and testing data (green dots) are each fitted with a linear regression line, demonstrating a negative correlation where increased mean distance corresponds to decreased accuracy. The steeper slope of the training data fit (-0.806) compared to the testing data fit (-0.677) reflects the greater accuracy and more compact cluster obtained from the correct test predictions compared to the cluster obtained from correct training predictions.}
%     \label{fig:MNIST_Classification_Train_Test_Accuracy_Mean_Distance_to_Centroid_Linear_Fit}
% \end{figure}

% function call
% plot_digit_averages(train_correct_predictions, train_incorrect_predictions, color1='skyblue', color2='lightcoral', data="Training Data")

\begin{figure}[h]
    \centering
    \includegraphics[width=0.95\columnwidth]{Figures/MNIST_Softmax_Averages_Training.png}
    \caption{Zoom in for detail. Average Softmax Probabilities for Correctly and Incorrectly Classified Digits in the MNIST Training Dataset}
    \label{fig:MNIST_Softmax_Averages_Training}
\end{figure}

% Plot generated with function:
% plot_accuracy_vs_distance_linear_fit(correct_train_distances, train_class_accuracies, correct_test_distances, test_class_accuracies)
% mnist_cnn_eval_saved_softmax_output.py

% Both fits reinforce the concept that compact clusters lead to better classification performance. ???
% Do they ???

These insights are crucial for informing the refinement of the classification model. They indicate that efforts to reduce within-class variance, potentially through data augmentation or more sophisticated feature extraction, could result in improved accuracy. Furthermore, understanding the different sensitivities in training versus testing can help diagnose overfitting and guide the development of more generalisable models.

In summary, the linear relationship elucidated by the fitted functions provides quantitative backing for the intuitive notion that tighter clusters (with respect to the centroid) lead to better classification performance. It reinforces the importance of cluster cohesion as an objective metric in assessing and improving classifier models, particularly in the realm of handwritten digit recognition.

% d2c = calculate_distances_to_centroids(train_correct_predictions, centroids)
% uel, ucnts = np.unique(d2c[:, 1], return_counts=True)
% ucnts
% array([5890, 6704, 5859, 6019, 5755, 5339, 5884, 6199, 5581, 5844])




% Figure \ref{fig:MNIST_Softmax_Averages_Training} shows the average softmax probabilities for each digit class (0 to 9) in the MNIST training dataset, separated into correctly classified instances (top row) and incorrectly classified instances (bottom row). The probabilities are displayed on a logarithmic scale. For correctly classified digits, the highest average probability is observed for the corresponding true digit class, indicating strong confidence in the correct predictions. In contrast, for incorrectly classified digits, the average probabilities are more evenly distributed across different digit classes, suggesting lower confidence and potential confusion between similar-looking digits. The plot provides insights into the model's behavior and the challenges in accurately classifying certain digit classes.
% Figure \ref{fig:MNIST_Softmax_Averages_Testing} is the corresponding plot for the MNIST testing dataset.

% % function call
% % plot_digit_averages(test_correct_predictions, test_incorrect_predictions, color1='lightgreen', color2='lightcoral', data="Testing Data")
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.99\columnwidth]{Figures/MNIST_Softmax_Averages_Testing.png}
%     \caption{Zoom in for detail. Average Softmax Probabilities for Correctly and Incorrectly Classified Digits in the MNIST Testing Dataset.}
%     \label{fig:MNIST_Softmax_Averages_Testing}
% \end{figure}

% \begin{table}[htbp]
% \centering
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
% \tiny
% \small
% idx & \multicolumn{3}{c|}{Train} & \multicolumn{3}{c|}{Test} & \multicolumn{3}{c|}{Train-Test} \\
% \hline
%  & Cnt & Ttl & Opct & Cnt & Ttl & Opct & Cnt & Ttl & Opct \\
% \hline
% 0 & 9 & 5890 & 0.15\% & 0 & 977 & 0.00\% & 1 & 5890 & 0.02\% \\
% 1 & 0 & 6704 & 0.00\% & 0 & 1129 & 0.00\% & 0 & 6704 & 0.00\% \\
% 2 & 7 & 5859 & 0.12\% & 0 & 1015 & 0.00\% & 2 & 5859 & 0.03\% \\
% 3 & 15 & 6019 & 0.25\% & 2 & 998 & 0.20\% & 5 & 6019 & 0.08\% \\
% 4 & 0 & 5755 & 0.00\% & 0 & 972 & 0.00\% & 0 & 5755 & 0.00\% \\
% 5 & 23 & 5339 & 0.43\% & 0 & 883 & 0.00\% & 0 & 5339 & 0.00\% \\
% 6 & 12 & 5884 & 0.20\% & 0 & 941 & 0.00\% & 4 & 5884 & 0.07\% \\
% 7 & 6 & 6199 & 0.10\% & 0 & 1009 & 0.00\% & 2 & 6199 & 0.03\% \\
% 8 & 137 & 5581 & 2.45\% & 2 & 934 & 0.21\% & 7 & 5581 & 0.13\% \\
% 9 & 14 & 5844 & 0.24\% & 0 & 980 & 0.00\% & 10 & 5844 & 0.17\% \\
% \hline
% \end{tabular}
% \caption{Comparison of centroid distances between correct and incorrect predictions}
% \label{tab:centroid_distance_overlap}
% \end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% CIFAR10 BOXPLOTS SIDE BY SIDE %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Plot generated with function call
% boxplots_side_by_side_x2(d2c_train_correct, 
%                         d2c_train_incorrect, 
%                         d2c_test_correct_train_centroids, 
%                         d2c_test_incorrect_train_centroids, 
%                         labels=class_labels,
%                         save=True, 
%                         debug=True,
%                         title1='Training Dataset Distribution of Distances to Centroids',
%                         title2='Testing Dataset Distribution of Distances to Centroids',
%                         xlabel1='CIFAR10 Training Dataset Class Prediction',
%                         xlabel2='CIFAR10 Testing Dataset Class Prediction',
%                         ylabel1='Distance to Centroid (Logarithmic Scale)',
%                         ylabel2='',
%                         filename='CIFAR10_boxplots_side_by_side_x2.png',
%                         figsize=(20, 5)
%                     )

% \begin{figure*}[h]
%     \centering
%     \includegraphics[width=0.99\textwidth]{Figures/CIFAR10_boxplots_side_by_side_x2.png}   \captionsetup{justification=raggedright,singlelinecheck=false}
%     \caption{Distribution of Distances to Centroids for Correctly and Incorrectly Classified Instances in Training and Testing CIFAR Data, where training data is on the left and testing data is displayed on the right. Distances are shown on a logarithmic scale. Note, centroids are for the correctly classified training examples, for both training and testing dataset.}
%     \label{fig:CIFAR10_boxplots_side_by_side_x2}
% \end{figure*}

% In figure \ref{fig:CIFAR10_boxplots_side_by_side_x2} note there are no incorrect classifications for class frog in the testing dataset.

%%%%%%%%%%%%%%%%%
% OVERLAP TABLE %
%%%%%%%%%%%%%%%%%

% Table generated with function call:
% centroid_distance_overlap_latex(d2c_train_correct, d2c_train_incorrect, d2c_test_correct, d2c_test_incorrect)
% \begin{table}[htbp]
% \centering
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% Digit & \multicolumn{3}{c|}{Train Data - Train Centroids} & \multicolumn{3}{c|}{Test Data - Train Centroids} \\
% \hline
%  & Count & Total & Overlap & Count & Total & Overlap \\
% \hline
% 0 & 2 & 5890 & 0.03\% & 1 & 977 & 0.10\% \\
% 1 & 0 & 6704 & 0.00\% & 0 & 1129 & 0.00\% \\
% 2 & 1 & 5859 & 0.02\% & 0 & 1015 & 0.00\% \\
% 3 & 3 & 6019 & 0.05\% & 1 & 998 & 0.10\% \\
% 4 & 0 & 5755 & 0.00\% & 0 & 972 & 0.00\% \\
% 5 & 5 & 5339 & 0.09\% & 0 & 883 & 0.00\% \\
% 6 & 2 & 5884 & 0.03\% & 1 & 941 & 0.11\% \\
% 7 & 2 & 6199 & 0.03\% & 0 & 1009 & 0.00\% \\
% 8 & 12 & 5581 & 0.22\% & 1 & 934 & 0.11\% \\
% 9 & 1 & 5844 & 0.02\% & 0 & 980 & 0.00\% \\
% \hline
% Totals & 28 & 59074 & 0.05\% & 4 & 9838 & 0.04\% \\
% \hline
% \end{tabular}
% \caption{Counts of correctly classified training and testing image predictions with distance to centroids equal or above error threshold $\varepsilon_{\text{th}}(i)$ where $i$ is the digit class}
% \label{tab:centroid_distance_overlap}
% \end{table}

% Table \ref{tab:centroid_distance_overlap} show the counts of correctly classified training and testing examples that are assigned a  By choosing the $\varepsilon_{\text{th}}(i)$ the accuracy.

% \begin{figure}[h]
%     \centering
% \includegraphics[width=0.99\columnwidth]{Figures/plot_accuracy_decrements.png}
%     \caption{Zoom in for detail. Accuracy decrements}
%     \label{fig:plot_accuracy_decrements}
% \end{figure}

% Plot generated by function call
% single_plot_accuracy_decrements(accuracy_results, overall_results, save=True)
% \begin{figure}[h]
%     \centering    
%     \includegraphics[width=0.99\columnwidth]{Figures/single_plot_accuracy_decrements.png}
%     \caption{Single plot Accuracy decrements}   \label{fig:single_plot_accuracy_decrements}
% \end{figure}

%%%%%%%%%%%%%%%%%%%
% CIFAR10 RESULTS %
%%%%%%%%%%%%%%%%%%%

% \subsection{CIFAR10 Results}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% PLOT ALL TESTING DATASET CLASS ACCURACY DECREMENTS %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Plot generated with function call
% plot_accuracy_decrements(accuracy_results, 
                         % overall_results,
                         % labels=class_labels, 
                         % save=True, 
                         % x_label='Threshold Decrement Factor', 
                         % title='CIFAR10 Testing Dataset Class Prediction Accuracy vs Distance to Threshold Decrement Factor', 
                         % filename='CIFAR10_testing_plot_accuracy_decrements.png')

% \begin{figure}[h]
%     \centering
% \includegraphics[width=0.99\columnwidth]{Figures/CIFAR10_testing_plot_accuracy_decrements.png}
%     \caption{Zoom in for detail. Accuracy decrements for CIFAR10 testing data}
%     \label{fig:CIFAR10_testing_plot_accuracy_decrements}
% \end{figure}

% Figure \ref{fig:CIFAR10_testing_plot_accuracy_decrements} shows the expected accuracy decrement for the CIFAR10 training dataset as the threshold decreases in factors of 0.1.

% We train our neural network, and make a record of the class probability outputs, true class and predicted class. Figure \ref{fig:cifar10_combined_confusion_matrix}

% % plot produced with function call:
% % conf_matrix1, conf_matrix2 = display_misclassifications_side_by_side_cifar10(train_np, test_np, 10, 11, class_labels, 20, 7, True)
% \begin{figure}[h]
%     \centering   
%     \includegraphics[width=0.99\columnwidth]{Figures/cifar10_combined_confusion_matrix.png}
%     \caption{Please zoom in for detail. Confusion matrices for the CIFAR10 classification model on the training dataset (left) and testing dataset (right). The matrices display the true labels on the vertical axis and the predicted labels on the horizontal axis. The diagonal elements represent correctly classified instances, while the off-diagonal elements indicate misclassifications.}
%     \label{fig:cifar10_combined_confusion_matrix}
% \end{figure}

%%%%%%%%%%%%%%%
% LATEX TABLE %
%%%%%%%%%%%%%%%

% Table generated by function call
% centroid_distance_overlap_latex(d2c_train_correct, 
%                                 d2c_train_incorrect, 
%                                 d2c_test_correct, 
%                                 d2c_test_incorrect, 
%                                 labels=class_labels,
%                                 caption='CIFAR10 centroid distances overlap count for correct predictions above incorrect threshold'
%                             ) 

% \begin{table}[htbp]
% \centering
% \begin{tabular}{|c|c|c|c|c|c|c|}
% \hline
% Class & \multicolumn{3}{c|}{Train Data - Train Centroids} & \multicolumn{3}{c|}{Test Data - Train Centroids} \\
% \hline
%  & Count & Total & Overlap & Count & Total & Overlap \\
% \hline
% plane & 13 & 4252 & 0.31\% & 1 & 990 & 0.10\% \\
% auto & 1 & 4326 & 0.02\% & 0 & 989 & 0.00\% \\
% bird & 9 & 4216 & 0.21\% & 0 & 993 & 0.00\% \\
% cat & 20 & 4103 & 0.49\% & 2 & 973 & 0.21\% \\
% deer & 14 & 4255 & 0.33\% & 0 & 991 & 0.00\% \\
% dog & 11 & 4157 & 0.26\% & 1 & 967 & 0.10\% \\
% frog & 11 & 4310 & 0.26\% & 0 & 1000 & 0.00\% \\
% horse & 12 & 4223 & 0.28\% & 0 & 991 & 0.00\% \\
% ship & 11 & 4258 & 0.26\% & 0 & 998 & 0.00\% \\
% truck & 10 & 4251 & 0.24\% & 0 & 981 & 0.00\% \\
% \hline
% Totals & 112 & 42351 & 0.26\% & 4 & 9873 & 0.04\% \\
% \hline
% \end{tabular}
% \caption{CIFAR10 centroid distances overlap count for correct predictions above incorrect threshold}
% \label{tab:centroid_distance_overlap}
% \end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Average Softmax Probabilities for Correctly and Incorrectly %
% Classified Classes in the CIFAR10 dataset                   %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Plot generated by function call
% single_plot_accuracy_decrements(accuracy_results, overall_results, labels=class_labels, dataset="CIFAR10", save=True)

% \begin{figure}[h]
%     \centering    
%     \includegraphics[width=0.99\columnwidth]{Figures/CIFAR10_single_plot_accuracy_decrements.png}
%     \caption{Single plot Accuracy decrements}   \label{fig:CIFAR10_single_plot_accuracy_decrements}
% \end{figure}

% Function call to generate plot
% plot_centroid_distance_bars(train_correct_predictions, 
                            % train_incorrect_predictions, 
                            % labels=class_labels, 
                            % color1='lightblue', 
                            % color2='lightcoral', 
                            % data="CIFAR10 Training Data", 
                            % save=True, 
                            % filename='CIFAR10_training_plot_centroid_distance_bars.png')

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.95\columnwidth]{Figures/CIFAR10_training_plot_centroid_distance_bars.png}
%     \caption{Zoom in for detail. Average Softmax Probabilities for Correctly and Incorrectly Classified Classes in the CIFAR10 Training Dataset}
%     \label{fig:CIFAR10_training_plot_centroid_distance_bars.png}
% \end{figure}

% Function call to generate plot
% plot_centroid_distance_bars(test_correct_predictions, 
%                             test_incorrect_predictions, 
%                             labels=class_labels, 
%                             color1='lightgreen', 
%                             color2='lightcoral', 
%                             data="CIFAR10 Testing Data", 
%                             save=True, 
%                             filename='CIFAR10_testing_plot_centroid_distance_bars.png')

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.95\columnwidth]{Figures/CIFAR10_testing_plot_centroid_distance_bars.png}
%     \caption{Zoom in for detail. Average Softmax Probabilities for Correctly and Incorrectly Classified classes in the CIFAR10 Testing Dataset}
%     \label{fig:CIFAR10_testing_plot_centroid_distance_bars.png}
% \end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% COMBINED CIFAR10 MNIST ACCURACY VS MEAN %
% CLASS PREDICTION DISTANCE TO THRESHOLD  %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Plot created by joining plots created by plot_accuracy_vs_distance_linear_fit

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.99\columnwidth]{Figures/Combined_CIFAR10_MNIST_single_plot_accuracy_decrements.png}
%     \caption{Please zoom in for detail. Expected accuracy decrease as a result of threshold decrease. MNIST data is on the left, CIFAR is on the right. Class predictions with softmax distance to class centroid below the class threshold are expected to be 100\% accurate, class predictions with distances equal or greater than threshold are then left to human judgement.}
% \label{fig:Combined_CIFAR10_MNIST_single_plot_accuracy_decrements.png}
% \end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% COMBINED CIFAR10 MNIST ACCURACY VS MEAN %
% CLASS PREDICTION DISTANCE TO CENTROID   %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Plot created manually from MNIST and CIFAR10 plots created by function plot_accuracy_vs_distance_linear_fit
% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.99\columnwidth]{Figures/Combined_CIFAR10_MNIST_Classification_Train_Test_Accuracy_Mean_Distance_to_Centroid_Linear_Fit.png}
%     \caption{Zoom in for detail. Expected accuracy based on class prediction distance from centroid. MNIST fit is on the left, CIFAR10 is on the right.}
% \label{fig:Combined_CIFAR10_MNIST_Classification_Train_Test_Accuracy_Mean_Distance_to_Centroid_Linear_Fit.png}
% \end{figure}

%Combined_CIFAR10_MNIST_Classification_Train_Test_Accuracy_Mean_Distance_to_Centroid_Linear_Fit.png




==> Archive/06-Discussion.tex <==
%%%%%%%%%%%%%%
% DISCUSSION %
%%%%%%%%%%%%%%

\section{Discussion}

% note what we trying to quantify is, for every digit, how many of the testing examples are further from the training centroid than the incorrect prediction nearest to the training centroid.

% Yes, that makes perfect sense. We are trying to quantify, for each digit, the number of testing examples that are further away from the training centroid compared to the incorrect prediction that is nearest to the training centroid.

% In other words, we want to determine, for each digit:

%     The minimum distance from the training centroid among all the incorrect predictions in the training data. This distance serves as the threshold for considering a prediction as "safe" or "unsafe".
%     The number of testing examples (both correct and incorrect predictions) that have a distance greater than or equal to this minimum incorrect distance threshold.

% By doing this, we can identify the testing examples that are more likely to be incorrectly predicted based on their distance from the training centroid. If a testing example has a distance greater than or equal to the minimum incorrect distance threshold, it suggests that it is further away from the centroid compared to the nearest incorrect prediction in the training data. Therefore, it can be considered an "unsafe" prediction and deferred to a human for manual review.

% On the other hand, testing examples with distances less than the minimum incorrect distance threshold are considered "safe" predictions, as they are closer to the centroid than the nearest incorrect prediction in the training data.

% This approach allows us to quantify the number of testing examples that are potentially prone to incorrect predictions based on their distance from the training centroid, using the nearest incorrect prediction in the training data as a reference point.


% The assumption is that at run time, the (correctly classified examples) softmax centroids will be used to quantify prediction robustness. If the distance to the class centroid is below threshold $t_c$ the prediction used, if the distance is greater or equal to $t_c$ the prediction is discarded and the decision is deferred to a human.

==> Archive/08-Acknowledgements.tex <==
%%%%%%%%%%%%%%%%%%%%
% ACKNOWLEDGEMENTS %
%%%%%%%%%%%%%%%%%%%%

\begin{ack}
By using the \texttt{ack} environment to insert your (optional) 
acknowledgements, you can ensure that the text is suppressed whenever 
you use the \texttt{doubleblind} option. In the final version, 
acknowledgements may be included on the extra page intended for references.
\end{ack}

==> Archive/09-TheStoryWeAreTryingToTell.tex <==
Results

1. How we trained our networks OK
2. The confusion matrices for MNIST - OK
3. The stats table - OK

4. The "overlap" table
    We'll put this one after the boxplots
5. The boxplots OK

6. The Linear Fits OK
    We show how the trained neural network model achieves higher predictive accuracy for classes that have lower softmax distance to their respective class centroids, compared to classes for which the model has lower predictive accuracy.
    
5. The accuracy vs distance to kernel plots



8. The Bar charts


===================

IF POSSIBLE

1. In the "overlap" tables, also maybe add a count of incorrect predictions that are equal or below the maximum distance to centroids of correct predictons.

2. Move MNIST confusion matrix to supplementary material 


==> Archive/leftovers.tex <==
% from results

In this section we would like to show our results. It could be that we have too many to form a cohesive story.

\subsection{The PerMINST Dataset}

We put in quite a bit of work to create the PerMINST dataset, which contains the original MNIST plus perturbations. This could be a selling point, as we are setting a benchmark. On the other hand, we might want to leave this for a second paper, and just focus on MNIST/CIFAR for now, and our clustering algorithm. TBD. The discussion around what MNIST is could be dropped or moved to "Supplementary Materials" / Appendix session.

The MNIST dataset, a cornerstone in the field of machine learning, serves as a benchmark for evaluating the performance of algorithms in the domain of handwritten digit recognition. Comprising a collection of 70,000 grayscale images, each of 28x28 pixel resolution, the dataset is divided into two distinct sets: a training set containing 60,000 examples, and a test set with 10,000 examples (\cite{LeCun1998}). Each image within the dataset is associated with a label from 0 to 9, corresponding to the digit it represents.

This dataset has been instrumental in facilitating advancements in machine learning, particularly in the development and evaluation of algorithms capable of performing classification tasks. Its widespread adoption can be attributed to several factors, including the simplicity of the task it presents and its suitability for use in benchmarking the performance of various learning algorithms, ranging from simple linear classifiers to more complex deep learning models.

A key feature of the MNIST dataset is its pre-processing stage, where the digits have been size-normalized and centered in a fixed-size image. This pre-processing reduces the variability unrelated to digit identity, allowing researchers to focus on the algorithmic challenge of digit recognition rather than on the preprocessing steps.

The significance of the MNIST dataset in the realm of machine learning research is well-documented, with \cite{LeCun1998} providing an extensive overview of the dataset's creation, characteristics, and its role in fostering advancements in the field.

This foundational dataset has not only enabled the comparison of algorithmic performance in a standardized setting but has also contributed to the proliferation of research in neural networks, serving as a pivotal benchmark for innovations in the field.

% Dataset description

The MNIST dataset is comprised of two main components: image files and label files, structured as follows:

\begin{itemize}
    \item \textbf{Training Set Images:} Contains 60,000 training examples.
    \item \textbf{Test Set Images:} Contains 10,000 test examples.
    \item Each image is encoded as a 28x28 pixel grid, summing up to 784 pixels per image. Each pixel represents a grayscale intensity, with 0 indicating white and 255 denoting black.
\end{itemize}

The structure of the image files is detailed below:
\begin{enumerate}
    \item \textbf{Magic Number:} The first 4 bytes signify a magic number (2051) that identifies the file format.
    \item \textbf{Number of Images:} The following 4 bytes denote the count of images, encoded as a 32-bit integer.
    \item \textbf{Rows:} The subsequent 4 bytes illustrate the number of rows (28) per image, encoded as a 32-bit integer.
    \item \textbf{Columns:} The next 4 bytes depict the number of columns (28) per image, encoded as a 32-bit integer.
    \item \textbf{Pixel Values:} The remainder of the file is populated with pixel values in row-major order, with each image delineated sequentially in the file. Each pixel value is stored as an unsigned byte, representing the pixel's intensity.
\end{enumerate}

and label files:
\begin{itemize}
    \item \textbf{Training Set Labels:} Comprises 60,000 labels corresponding to the training images.
    \item \textbf{Test Set Labels:} Comprises 10,000 labels corresponding to the test images.
    \item Each label is a single byte signifying the digit (0 through 9) that the corresponding image represents.
\end{itemize}

The structure of the label files is detailed below:
\begin{enumerate}
    \item \textbf{Magic Number:} The first 4 bytes signify a magic number (2049) that identifies the file format.
    \item \textbf{Number of Items:} The following 4 bytes denote the count of labels, encoded as a 32-bit integer.
    \item \textbf{Labels:} The remainder of the file contains label values, stored as unsigned bytes, with each label corresponding to the image of the same index in the image file.
\end{enumerate}

This standardized format ensures the MNIST dataset's compatibility with a wide array of machine learning models, particularly facilitating research in image classification and handwriting recognition.

\begin{table}[h]
\centering
{\footnotesize
\begin{tabular}{|l|l|r|r|}
\hline
\textbf{Type}             & \textbf{File Name}                       & \textbf{Size (B)} & \textbf{Cnt} \\ \hline
Train Images & \texttt{train-images-idx3-ubyte} & 47040016           & 60k \\
Train Labels & \texttt{train-labels-idx1-ubyte} & 60008             & 60k \\
Test Images  & \texttt{t10k-images-idx3-ubyte}  & 7840016           & 10k \\
Test Labels  & \texttt{t10k-labels-idx1-ubyte}  & 10008              & 10k \\ \hline
\end{tabular}
\caption{MNIST Dataset Files, file sizes in bytes and image/label count}
} % end tiny font
\label{table:mnist_files_b}
\end{table}
The header for the train-images-idx3-ubyte training image file looks like:
\begin{verbatim}
0000 0803 0000 ea60 0000 001c 0000 001c
\end{verbatim}
While the header for train-labels-idx1-ubyte the training label file looks like:
\begin{verbatim}
0000 0801 0000 ea60 0500 0401 0902 0103
\end{verbatim}

Where hex \textbf{0000 0803} is the magic number 2051 (images), and hex \textbf{0000 0801} is the magic number 2049 (labels), hex \textbf{0000 ea60}, 60,000 decimal, is the number of examples in the dataset, and hex \textbf{0000 001c}, decimal 28, is the number of rows, and columns, in every image. Therefore the number of bytes in train-images-idx3-ubyte is $4 * 4 + 60000 * 28 * 28 = 47,040,016$.

The first image in the training dataset can be obtained by offsetting the first 16 bytes (magic number, number of images, row size and column size) and taking the next 784 bytes, then splitting the array into 28 rows.


\begin{figure}[h]
    \centering
    \includegraphics[width=0.95\columnwidth]{Figures/MNIST_5_with_histogram.png}
    \caption{MNIST digit 5 and its pixel value distribution histogram.}
    \label{fig:mnist_5_histogram}
\end{figure}
As shown in Figure~\ref{fig:mnist_5_histogram}, the MNIST digit 5 is displayed alongside its pixel value distribution histogram where the pixel values range from 0 to 255. Figure~\ref{fig:mnist_0_histogram} shows the second image (zero) in the MNIST training dataset.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.95\columnwidth]{Figures/MNIST_0_with_histogram.png}
    \caption{MNIST digit 0 and its pixel value distribution histogram.}
    \label{fig:mnist_0_histogram}
\end{figure}

From the training labels dataset, it can be seen that by offsetting the magic number and the number of labels, represented by 4 bytes each, the following bytes represent the labels, that is, the first two labels are "05 and "00", matching figures \ref{fig:mnist_5_histogram} and \ref{fig:mnist_0_histogram}.

\subsection{Creating the "noisy" MNIST dataset}

To augment the research on image recognition robustness, we propose the creation of an enhanced training and testing dataset derived from the original MNIST dataset. This new dataset will incorporate a variety of perturbations to the original images, aiming to simulate real-world conditions where image data may not be ideal. Specifically, we will introduce noise to the images using 12 distinct functions designed to add perturbations, categorized as follows:

\begin{enumerate}
    \item \textbf{Pixel Intensity Adjustment:}
    \begin{itemize}
        \item Brightness
        \item Contrast
    \end{itemize}
    \item \textbf{Blurring:}
    \begin{itemize}
        \item Defocus Blur
        \item Motion Blur
        \item Zoom Blur
    \end{itemize}
    \item \textbf{Noise:}
    \begin{itemize}
        \item Gaussian Noise
        \item Impulse Noise
        \item Shot Noise
    \end{itemize}
    \item \textbf{Weather:}
    \begin{itemize}
        \item Fog
        \item Frost
        \item Snow
    \end{itemize}
    \item \textbf{Special Effects:}
    \begin{itemize}
        \item Pixelation
    \end{itemize}
\end{enumerate}

Each image in the original dataset will undergo transformation by one or more of these perturbation methods, resulting in a companion image that retains the original label but exhibits the added noise or effect. The new dataset will consist of pairs of images: the clean (original) and the noisy (perturbed) versions. To facilitate distinction and subsequent analysis, labels will be appended to denote the image type: "00" for clean/original images and "01" for noisy/perturbed images. This dual dataset structure will enable comprehensive evaluation of machine learning models' performance in recognizing digits under varied conditions, thereby enhancing the robustness of our image recognition pipeline.

% Applying noise

To generate our new dataset, we write to a binary file named perturbed-train-images-idx3-ubyte, where the first 16 bytes are:
\begin{verbatim}
0000 0803 0001 d4c0 0000 001c 0000 001c    
\end{verbatim}
Where 0001 d4c0 hex is 120000 decimal, the size of the new training dataset, twice the size of the original dataset.

We make a random selection of a perturbation type, and a perturbation level ranging from 0 to 9, and apply the perturbation to the image.

Figures \ref{fig:MNIST_4_clean_with_histogram} and \ref{fig:MNIST_4_noisy_with_histogram} show digit 4 with no noise and zoom blur level 8 applied.
\begin{figure}[h]
    \centering
    \includegraphics[width=0.95\columnwidth]{Figures/MNIST_4_clean_with_histogram.png}
    \caption{MNIST digit 4 with no noise.}
    \label{fig:MNIST_4_clean_with_histogram}
\end{figure}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.95\columnwidth]{Figures/MNIST_4_noisy_with_histogram.png}
    \caption{MNIST digit 4 with Zoom Blur level 8.}
    \label{fig:MNIST_4_noisy_with_histogram}
\end{figure}

% file to generate images is
% https://colab.research.google.com/drive/1s-KBSwUtT7tp280iLi8KgyHk4zThDnKD#scrollTo=OMq-a-wuKqR0
% MNIST-Dataset.ipynb

The process can be describe like so:

\begin{algorithm}
\caption{MNIST Perturbation Algorithm}
\label{alg:mnist_perturbation_algorithm}
\begin{algorithmic}[1]
\Procedure{createFiles}{}
    \State Open images.bin as binary write
    \State Open labels.bin as binary write
    \State Open perturbations.bin as binary write
\EndProcedure

\Procedure{saveImage}{image, file}
    \State Write image to file
\EndProcedure

\Procedure{saveLabel}{label, file}
    \State Write label to file as a single byte
\EndProcedure

\Procedure{savePerturbation}{perturbationCode, file}
    \State Write perturbationCode to file as bytes
\EndProcedure

\Procedure{main}{}
    \State createFiles()
    \For{each image in MNIST}
        \State saveImage(originalImage, images.bin)
        \State saveLabel(0x00, labels.bin)
        \State savePerturbation(0xFFFF, perturbations.bin)
        \State perturbedImage = applyRandomPerturbation(originalImage)
        \State saveImage(perturbedImage, images.bin)
        \State saveLabel(0x01, labels.bin)
        \State perturbationCode = getPerturbationCode()
        \State savePerturbation(perturbationCode, perturbations.bin)
    \EndFor
\EndProcedure
\end{algorithmic}
\end{algorithm}

We apply the same process to training and testing datasets, and end up with 6 files as shown in Table \ref{table:mnist_perturbed_files_b}.

% \begin{table}[h]
% \centering
% \begin{tabular}{|l|l|r|r|}
% \hline
% \textbf{Type}             & \textbf{File Name}                          & \textbf{Size (B)} & \textbf{Count} \\ \hline
% Perturbed Training Images  & \texttt{perturbed-train-images-idx3-ubyte}    & TBA               & 120000 \\                            
% Perturbed Training Labels  & \texttt{perturbed-train-labels-idx1-ubyte}    & TBA               & 120000 \\                            
% Perturbation Training Levels  & \texttt{perturbation-train-levels-idx0-ubyte} & TBA               & 120000 \\
% Perturbed Testing Images   & \texttt{t20k-perturbed-images-idx3-ubyte}     & TBA               & 20000 \\                            
% Perturbed Testing Labels   & \texttt{t20k-perturbed-labels-idx1-ubyte}     & TBA               & 20000 \\  
% Perturbation Testing Levels   & \texttt{t20k-perturbation-levels-idx0-ubyte}     & TBA               & 20000 \\ \hline                 
% \end{tabular}
% \caption{Perturbed MNIST (PMNIST) Dataset Files, file sizes in bytes and image/label count}
% \label{table:mnist_perturbed_files_b}
% \end{table}

\begin{table}[h]
\centering
{\tiny
\begin{tabular}{|l|l|l|r|r|}
\hline
\textbf{ID} & \textbf{Type}                   & \textbf{File Name}                                   & \textbf{Size (B)} & \textbf{Count} \\ \hline
1 & Perturbed Training Images       & \texttt{perturbed-train-images-idx3-ubyte}    & TBA               & 120000 \\
2 & Perturbed Training Labels       & \texttt{perturbed-train-labels-idx1-ubyte}    & TBA               & 120000 \\
3 & Perturbation Training Levels    & \texttt{perturbation-train-levels-idx0-ubyte} & TBA               & 120000 \\
4 & Perturbed Testing Images        & \texttt{t20k-perturbed-images-idx3-ubyte}     & TBA               & 20000 \\
5 & Perturbed Testing Labels        & \texttt{t20k-perturbed-labels-idx1-ubyte}     & TBA               & 20000 \\
6 & Perturbation Testing Levels     & \texttt{t20k-perturbation-levels-idx0-ubyte}  & TBA               & 20000 \\ \hline
\end{tabular}
} % End of \small
\caption{Perturbed MNIST (PMNIST) Dataset Files, file sizes in bytes and image/label count}
\label{table:mnist_perturbed_files_b}
\end{table}

Where the additional files are perturbation-train-levels-idx0-ubyte and t20k-perturbation-levels-idx0-ubyte that contain the perturbation types and levels, stored contiguously in one byte values. As per the algorithm described in \ref{alg:mnist_perturbation_algorithm}, We start by opening the binary files. We then iterate over every image in the MNIST dataset. We apply a random perturbation and perturbation level to the image, writing the original and perturbed image to the new PMNIST dataset (ID 1). We write the image label twice (ID 2), once with value 0 indicating the image is noise-free, and once with value 1 indicating the image is perturbed, aligning with the saved images and finally we write the perturbation key and level (ID 3). We repeat the steps for the testing dataset, obtaining 3 additional files (IDs 4, 5 and 6).

\subsection{Validating predictions}

We consider the neural network output, a vector containing values summing up to 1. That is a probability distribution obtained from normalising the logits output by the network, i.e. the raw prediction values, where the highest value index corresponds to the predited class e.g. given the Softmax function output [0.01, 0.01, 0.01, 0.01, 0.9, 0.01, 0.01, 0.01, 0.01, 0.01], the predicted class is the number 4, given the highest value found in index number five of the vector, where the first position corresponds to the prediction confidence the image given to the network is zero, and the last is the same for number 9. The softmax function, as discussed earlier, is then applied to the logits to convert them into a valid probability distribution:

\begin{equation}
p_i = \text{softmax}(z_i) = \frac{e^{z_i}}{\sum_{j=1}^{K} e^{z_j}}
\end{equation}

Mathematically, given an input image $\mathbf{x}$, the neural network computes a linear transformation followed by a non-linear activation function in each layer. The output of the final layer, before applying the softmax activation, is the logit vector $\mathbf{z} = (z_1, z_2, \dots, z_K)$, where $K$ is the number of classes (10 in the case of MNIST) (\cite{goodfellow2016deep}).

he output of the final layer, before applying the softmax activation, is the logit vector $\mathbf{z} = (z_1, z_2, \dots, z_K)$, where $K$ is the number of classes (10 in the case of MNIST) \cite{goodfellow2016deep}.

The relationship between logits and probabilities can be expressed as follows:

\begin{equation}
z_i = \log \frac{p_i}{1 - p_i}
\end{equation}

where $z_i$ is the logit for class $i$, and $p_i$ is the probability of the input belonging to class $i$. The logits are logarithms of the odds ratios, representing the log-likelihood of the input belonging to a particular class compared to the other classes (\cite{bishop2006pattern}).


In other words, we want to determine, for each digit:

    The minimum distance from the training centroid among all the incorrect predictions in the training data. This distance serves as the threshold for considering a prediction as "safe" or "unsafe".
    The number of testing examples (both correct and incorrect predictions) that have a distance greater than or equal to this minimum incorrect distance threshold.

By doing this, we can identify the testing examples that are more likely to be incorrectly predicted based on their distance from the training centroid. If a testing example has a distance greater than or equal to the minimum incorrect distance threshold, it suggests that it is further away from the centroid compared to the nearest incorrect prediction in the training data. Therefore, it can be considered an "unsafe" prediction and deferred to a human for manual review.

On the other hand, testing examples with distances less than the minimum incorrect distance threshold are considered "safe" predictions, as they are closer to the centroid than the nearest incorrect prediction in the training data.

This approach allows us to quantify the number of testing examples that are potentially prone to incorrect predictions based on their distance from the training centroid, using the nearest incorrect prediction in the training data as a reference point.


The assumption is that at run time, the (correctly classified examples) softmax centroids will be used to quantify prediction robustness. If the distance to the class centroid is below threshold $t_c$ the prediction used, if the distance is greater or equal to $t_c$ the prediction is discarded and the decision is deferred to a human.

We consider the neural network output, a vector containing values summing up to 1. That is a probability distribution obtained from normalising the logits output by the network, i.e. the raw prediction values, where the highest value index corresponds to the predited class e.g. given the Softmax function output [0.01, 0.01, 0.01, 0.01, 0.9, 0.01, 0.01, 0.01, 0.01, 0.01], the predicted class is the number 4, given the highest value found in index number five of the vector, where the first position corresponds to the prediction confidence the image given to the network is zero, and the last is the same for number 9. The softmax function, as discussed earlier, is then applied to the logits to convert them into a valid probability distribution:

\begin{equation}
p_i = \text{softmax}(z_i) = \frac{e^{z_i}}{\sum_{j=1}^{K} e^{z_j}}
\end{equation}

Mathematically, given an input image $\mathbf{x}$, the neural network computes a linear transformation followed by a non-linear activation function in each layer. The output of the final layer, before applying the softmax activation, is the logit vector $\mathbf{z} = (z_1, z_2, \dots, z_K)$, where $K$ is the number of classes (10 in the case of MNIST) (\cite{goodfellow2016deep}).

he output of the final layer, before applying the softmax activation, is the logit vector $\mathbf{z} = (z_1, z_2, \dots, z_K)$, where $K$ is the number of classes (10 in the case of MNIST) \cite{goodfellow2016deep}.

The relationship between logits and probabilities can be expressed as follows:

\begin{equation}
z_i = \log \frac{p_i}{1 - p_i}
\end{equation}

where $z_i$ is the logit for class $i$, and $p_i$ is the probability of the input belonging to class $i$. The logits are logarithms of the odds ratios, representing the log-likelihood of the input belonging to a particular class compared to the other classes (\cite{bishop2006pattern}).

% To facilitate the analysis of centroid distances for incorrectly predicted CIFAR-10 and MNIST classes, we have developed an algorithm that efficiently finds the minimum distance to the centroid for each digit class. By organizing the minimum distances and their corresponding labels in a structured array, researchers and practitioners can easily access and interpret this information. The algorithm leverages array arithmetic and the min function to streamline the computation process and provide a concise representation of the results.

% The motivation behind creating this algorithm is to provide a tool for gaining insights into the behavior of classifiers. By identifying the minimum centroid distances for incorrectly predicted classes, researchers can investigate the characteristics of misclassified samples, detect potential outliers or ambiguous cases, and develop strategies for determining what predictions should be deferred to human judgement. This algorithm contributes to the broader goal of advancing machine learning techniques and enhancing the accuracy and reliability of classifiers.


\subsection{Clustering}
To initialise the centroids for K-Means clustering with 10 clusters, where each cluster represents a digit from the MNIST dataset, we leverage the information from the probability distribution of the correct predictions.

The resulting centroids array will have shape (10, 10), where each row represents a centroid for a specific digit. The values in each row correspond to the average probability distribution of the correct predictions for that digit.

To find the centroids, we use:

The algorithm starts with the Require statement, specifying the input correct\_preds array of shape $(n, 12)$, where $n$ is the number of correct predictions.
The Ensure statement specifies the output centroids array of shape $(10, 10)$, which will store the initialised centroids for each digit.
In line 1, we extract the probability distribution for each digit by selecting the first 10 columns of correct\_preds and store it in the prob\_dist array, where column 11 is the label and column 12 is the prediction, and both are the same for correct predictions.
In line 2, we initialise the centroids array with zeros of shape $(10, 10)$ to store the centroid for each digit.
We start a loop that iterates over each digit from 0 to 9.
In line 4, for each digit, we find the indices of rows in prob\_dist where the digit has the highest probability using \text{argmax}(prob\_dist, \text{axis}=1) == digit. This gives us the indices of rows that are most likely to represent the current digit, which is indeed the case since all predictions are correct.
In line 5, we compute the mean probability distribution for the selected rows using \text{mean}(prob\_dist[indices], \text{axis}=0). This gives us the centroid for the current digit.
In line 6, we assign the computed centroid to the corresponding row in the centroids array.
After the loop ends, we return the centroids array.

The resulting centroids array will have shape $(10, 10)$, where each row represents a centroid for a specific digit. The values in each row correspond to the average probability distribution of the correct predictions for that digit.

By initialising the centroids based on the probability distribution of correct predictions, we provide a good starting point for the K-Means algorithm. Each centroid will be initialised to represent the typical probability distribution for a specific digit class prediction, which helps the algorithm converge faster.

We define the error threshold $\varepsilon_{\text{th}}(i)$ as the closest distance to the class centroid for every incorrectly predicted digit $i$.



1. The procedure `FindMinDistances` takes a parameter `data`, which is a zero-indexed array of shape $(n, 2)$, where column 1 contains distances to centroids of incorrectly predicted MNIST dataset digits, and column 2 contains the incorrectly predicted digits (0 to 9).
2. We define an array `labels` containing the digits 0 to 9.
3. We create an empty array `thresh` of shape $(10, 2)$ to store the minimum distances and corresponding labels.
4. We iterate over the indices 0 to 9.
5. For each index `i`, we assign the corresponding label from `labels` to the variable `label`.
6. We use array arithmetic to find the minimum distance for the current label. The expression `data[data[:, 1] == label, 0]` selects the rows of `data` where the second column (index 1) is equal to the current `label`, and then selects the first column (index 0) of those rows. We apply the `min` function to find the minimum value among the selected distances.
7. We assign the minimum distance (`min\_dist`) to the first column of `thresh` at index `i`.
8. We assign the current `label` to the second column of `thresh` at index `i`.
9. After iterating over all labels, we return the `thresh` array containing the minimum distances and corresponding labels.

This modified algorithm uses array arithmetic to find the minimum distance for each label (digit) in a more concise and efficient manner. The `min` function is applied to the selected rows of `data` where the second column matches the current label, and the minimum distance is extracted from the first column of those rows. The resulting `thresh` array contains the minimum distances and their corresponding labels.

\subsection{Confusion Matrix Discussion 1}

The confusion matrices for the CIFAR-10 training and testing datasets provide insights into the performance of the classification model. In the training dataset, the model achieves high accuracy for most classes, as evidenced by the large values along the diagonal. However, there are some notable misclassifications, such as the confusion between the "cat" and "dog" classes, where 182 "cat" instances are misclassified as "dog," and 174 "dog" instances are misclassified as "cat." This suggests that the model may struggle to distinguish between these two visually similar classes.

Other misclassifications in the training dataset include the confusion between "bird" and "airplane," where 57 "bird" instances are misclassified as "airplane," and 33 "airplane" instances are misclassified as "bird." This indicates that the model may have difficulty differentiating between these two classes, possibly due to shared visual features such as wings or beaks.

In the testing dataset, the model's performance is generally lower compared to the training dataset, which is expected due to the model being evaluated on unseen data. The diagonal elements still show a high number of correctly classified instances for most classes, but the misclassifications are more pronounced. For example, the confusion between "cat" and "dog" persists, with 17 "cat" instances misclassified as "dog," and 29 "dog" instances misclassified as "cat." Additionally, there are misclassifications between "automobile" and "truck," where 10 "automobile" instances are misclassified as "truck," and 3 "truck" instances are misclassified as "automobile."

The color scale provides a visual cue for the severity of misclassifications. In the testing dataset, the darker off-diagonal elements highlight the more frequent misclassifications, such as the confusion between "cat" and "dog," and between "automobile" and "truck."

These confusion matrices suggest that while the model performs well overall, there are specific class pairs that are more challenging for the model to distinguish. Addressing these misclassifications may require further refinement of the model's architecture, additional training data for the problematic classes, or the use of techniques such as data augmentation or transfer learning to improve the model's generalization ability.

\subsection{Linear fit discussion 2}

The image presents two scatter plots that illustrate the relationship between classification accuracy and the mean class distance to a centroid for different datasets. The plot on the left shows the results for the MNIST dataset, while the plot on the right displays the findings for the CIFAR10 dataset.

In the MNIST plot, the training data, represented by green dots, exhibits a strong linear relationship between the mean class distance to the centroid and the classification accuracy. The linear fit for the training data is given by the equation: $Train Fit: -0.800*x + 1.009$. The test data, denoted by purple dots, also follows a linear trend, albeit with a slightly different slope and intercept, as described by the equation: $Test Fit: -0.677*x + 1.004$. These linear fits suggest that as the mean class distance to the centroid decreases, the classification accuracy tends to increase for both the training and test datasets.

Similarly, in the CIFAR10 plot, the training data (green dots) and test data (purple dots) demonstrate linear relationships between the mean class distance to the centroid and the classification accuracy. The linear fit for the training data is represented by the equation: $Train Fit: -1.237*x + 0.987$, while the test data fit is given by: $Test Fit: -1.412*x + 0.999$. As with the MNIST dataset, the negative slopes of the linear fits indicate that a decrease in the mean class distance to the centroid is associated with an increase in classification accuracy.

It is worth noting that the CIFAR10 dataset exhibits a steeper slope compared to the MNIST dataset, suggesting a stronger influence of the mean class distance to the centroid on the classification accuracy. Furthermore, the CIFAR10 data points appear to have a slightly larger spread around the linear fits, indicating more variability in the relationship between the two variables.

Overall, these findings underscore the importance of the mean class distance to the centroid in determining the classification accuracy of machine learning models. The linear relationships observed in both datasets provide valuable insights into the interplay between these two metrics and can guide researchers in developing more accurate and robust classification algorithms.

\subsection{Linear Fit discussion 3}

The image appears to contain two scatter plots, each with a linear fit line for both training and test data, displaying the relationship between classification accuracy and the mean distance to centroid for two datasets: MNIST and CIFAR-10.

For the MNIST dataset, the scatter plot indicates a negative correlation between mean class distance to centroid and classification accuracy. The linear fit for the training data is represented by the equation \( \text{Accuracy}_{\text{train}} = -0.806 \times \text{Mean Distance to Centroid} + 1.009 \), while the test data is described by \( \text{Accuracy}_{\text{test}} = -0.677 \times \text{Mean Distance to Centroid} + 1.004 \). These relationships suggest that, as the mean distance of class outputs to the centroid decreases, the classification accuracy improves. Notably, the training data exhibits a steeper slope, indicating a more pronounced effect as compared to the test data.

Similarly, for the CIFAR-10 dataset, the plot again shows a negative correlation. The linear fit for the training data follows \( \text{Accuracy}_{\text{train}} = -1.237 \times \text{Mean Distance to Centroid} + 0.987 \), whereas the test data is modeled by \( \text{Accuracy}_{\text{test}} = -1.412 \times \text{Mean Distance to Centroid} + 0.999 \). This trend is consistent with the MNIST results, where a smaller mean distance to centroid correlates with higher accuracy. Once more, the training data demonstrates a steeper slope, indicating a stronger relationship between the mean distance to centroid and classification accuracy during training.

The consistency of these negative correlations across both datasets and both training and test data supports the hypothesis that models with output probabilities clustered closer to the class centroid tend to achieve higher classification accuracies. The slopes of the linear fit for the training data are steeper than those for the test data in both datasets, which may suggest that the model's ability to minimize the distance to the centroid is more pronounced during the training phase, possibly due to overfitting or the model learning the training data distributions more closely than it can generalize to the test data. 

These findings may be indicative of the internal representations that the neural network learns during training, where classes that are more tightly clustered around a centroid in the feature space are easier for the model to discriminate, leading to higher classification accuracy. Further research could investigate the underlying causes of these clustering patterns and whether they can be leveraged to improve the generalizability of neural network models.


==> Sections/08-RejectionNote.tex <==
\section*{[ECAI-2024] Notification for submission \#1654}

Dear Daniel,

We regret to inform you that your submission entitled ``When to Trust Automated Predictions and When to Defer to Human Judgment?'' (\#1654) has not been accepted for publication at the 27th European Conference on Artificial Intelligence (ECAI-2024).

As for every edition of the conference, the reviewing process was thorough and highly selective. We received a total of 2,344 submissions and accepted 547 of them, corresponding to an acceptance rate of 23\%. The list of accepted papers will become available at the conference website next week.

Every submission was reviewed by at least three experts in the field. The initial reviews and your rebuttal (if you chose to submit one) were then discussed by those reviewers and a senior member of the programme committee, who summarised the outcome of the discussion in a brief metareview. In a small number of cases, additional experts were consulted during this discussion phase. Every discussion was monitored and every metareview approved by an area chair. You will find your final reviews both at the end of this message and on EasyChair. We hope that you will find the feedback received helpful.

You may want to consider submitting a revised version of your paper to one of the many exciting workshops associated with ECAI-2024. While some deadlines have passed already, several workshops have a fast-track option for papers rejected from the main conference. We will send you a separate message about this later today.

Either way, we would be delighted to see you in Santiago de Compostela this October, and for you to be part of the 50th anniversary of ECAI.

All the best,

Ulle Endriss and Francisco Melo\\
ECAI-2024 PC Chairs

Conference website: \url{https://www.ecai2024.eu/}\\
EasyChair: \url{https://easychair.org/conferences/?conf=ecai24}

Note that a copy of the review form used is available from the FAQ site.

\subsection*{SUBMISSION: 1654}
\textbf{TITLE: When to Trust Automated Predictions and When to Defer to Human Judgment?}

\subsection*{METAREVIEW}
The paper deals with the problem of estimating the confidence of a prediction in order to defer judgment to human experts, in particular in the case of distribution shifts.

While the problem is interesting, the reviewers raised a number of issues, notably the fact that the paper was not always very clear (they provided numerous examples to support this statement), and also the fact that it was unclear to which extent the experiments were specifically addressing the problem of distribution shift.

I would also add that since the classifiers is concerned with an estimation of the confidence of prediction, the paper should also be positioned with respect to the large uncertainty quantification literature and calibration methods existing around, that also try to achieve this purpose.

\subsection*{REVIEW 1}
\textbf{SUBMISSION:} 1654\\
\textbf{TITLE:} When to Trust Automated Predictions and When to Defer to Human Judgment?\\
\textbf{AUTHORS:} Daniel Sikar, Artur Garcez, Tillman Weyde, Robin Bloomfield and Kaleem Peeroo

\subsubsection*{Summary}
The paper presents a new method for assessing the reliability of neural network predictions under distribution shifts. The approach involves: clustering outputs, confidence metrics and definition of a safety threshold for predictions. The method is tested on the MNIST and CIFAR-10 datasets using different neural network models (Convolutional Neural Network and Vision Transformer). The results indicate that this metric is consistent across datasets and models, suggesting it can efficiently determine when automated decisions are reliable and when human intervention is necessary. The approach is also being evaluated in the CARLA simulator for self-driving scenarios under noisy conditions.

\subsubsection*{Strengths}
\begin{itemize}
    \item The paper is well structured and clear
    \item The assessment method proposed is presented in details, the algorithmic representations are also provided
    \item The approach is tested by using validated state of the art datasets
\end{itemize}

\subsubsection*{Weaknesses}
\begin{itemize}
    \item Figures are too small, by zooming in the digital version the details are clearly displayed, but not visible at all in the printed version. It would be useful providing readers with additional materials in which the figures are at the proper size.
\end{itemize}

\subsubsection*{Detailed comments}
The paper introduces a straightforward method to improve accuracy thresholding in image classification. The authors trained two different neural network models on two well-known datasets, demonstrating consistent results. They proposed a threshold to determine when predictions can be accepted. They also highlighted the need for human judgment since the threshold values are domain-specific and need experts intervention to balance automated decision.

The method is applied to self-driving car safety using the CARLA simulator, enhancing system safety by flagging scenarios where human judgment is needed, especially in out-of-distribution (OOD) situations. Additionally, the study explores using the softmax output as a training dataset for a multi-layer perceptron binary classifier, comparing this with their softmax distance approach and a regressor network to study optimal threshold values. The paper is well organized and in line with the conference topics.

\subsubsection*{Score}
SCORE: 4 (poor (fair attempt but too many concerns, so probably should be rejected))

\subsection*{REVIEW 2}
\textbf{SUBMISSION:} 1654\\
\textbf{TITLE:} When to Trust Automated Predictions and When to Defer to Human Judgment?\\
\textbf{AUTHORS:} Daniel Sikar, Artur Garcez, Tillman Weyde, Robin Bloomfield and Kaleem Peeroo

\subsubsection*{Summary}
The method proposed provides a way to estimate the confidence a model has in its classification results, in the shape of a softmax distance from a pre-computed cluster centroid. If the distance is above a threshold, the task is asked to a human to classify himself the sample. MNIST and CIFAR-10 have been used for this purpose, respectively with a simple MLP and a pre-trained ViT. The authors claim to measure the distribution shifts in the data, a problem with large impacts in the real-world settings (like under noisy weather conditions for self-driving cars).

\subsection*{Strengths}
\begin{itemize}
    \item The problem to address is clear, and is indeed related to real-world business concerns. It deserves to be treated as it is proposed here.
    \item Clustering classifier outputs and measure the distance between the inferred output and the cluster centroid is a good idea.
    \item Numerous evidences are provided, from the confusion matrices to the detailed distances distribution for all the classes.
\end{itemize}

\subsubsection*{Weaknesses}
\begin{itemize}
    \item It is not obvious to claim that the train and test sets of the mnist or cifar-10 come with distribution shifts. Both sets come from the same overall distribution, so the argument that the approach covers the distribution shift does not hold.
    \item Also, there is no comparison with competitor methods (as KL or MMD introduced in the 1st section), thus no way to understand the added value of the method.
    \item Datasets and models are not really representative of real-world settings, thus it is difficult to ensure that an autonomous safety system, like self-driving decision-making, can raise good results with this approach.
    \item It would be fine to see the clustering plots, in order to have a visual of the centroid positions, the spread in the clusters, the overlaps etc ...
    \item Sometimes difficult to follow (long sentences, repetitions, confusion, ...).
\end{itemize}

\subsubsection*{Detailed comments}
[Detailed comments omitted for brevity]

\subsubsection*{Questions for rebuttal}
\begin{enumerate}
    \item Why do you consider distribution shifts in the train and test set of MNIST or CIFAR-10?
    \item How does your method perform against other competitor ones?
    \item Why did you choose a CNN and a pre-trained ViT as classifiers (is there an explanation)?
\end{enumerate}

\subsubsection*{Score}
SCORE: 4 (poor (fair attempt but too many concerns, so probably should be rejected))

\subsubsection*{Comments added after rebuttal}
I'm not convinced by the author answers, who don't really explain neither the distribution shifts in the datasets, nor the comparison with the competitors. Therefore, no score change from my side.

\section*{REVIEW 3}
\textbf{SUBMISSION:} 1654\\
\textbf{TITLE:} When to Trust Automated Predictions and When to Defer to Human Judgment?\\
\textbf{AUTHORS:} Daniel Sikar, Artur Garcez, Tillman Weyde, Robin Bloomfield and Kaleem Peeroo

\subsubsection*{Summary}
The paper proposes a softmax method to quantify the reliability of CNN predictions.

\subsubsection*{Strengths}
\begin{itemize}
    \item Overall interesting topic
    \item 2 datasets
\end{itemize}

\subsubsection*{Weaknesses}
\begin{itemize}
    \item Lots of unclarity throughout the manuscript
    \item Figures (with important content) are not readable
    \item The introduction and conclusion do not well connect with the main part of the paper (non-stringent story)
\end{itemize}

\subsubsection*{Detailed comments}
[Detailed comments omitted for brevity]

\subsubsection*{Score}
SCORE: 2 (insufficient (arguably was not yet ready for submission))

\section{[ECAI-2024] Review Transfer Option for ECAI Satellite Workshops (deadline:  11 July 2024)}

Dear Daniel,

You are receiving this message as an author of a submission to ECAI-2024 that did not make it into the programme of the main conference.

ECAI-2024 will have a rich programme of satellite workshops and several of these workshops are offering a fast-track option for papers rejected from the main track. We can transfer your reviews to the organisers of one of the participating workshops, which will allow them to make a very fast decision.

If you are interested, please visit this page for full information:

https://bit.ly/ecai24transfer

The deadline for requesting the transfer of your reviews is next Thursday, 11 July 2024.

Make sure you also check the website of the workshop of your choice to find out how and by when to submit your paper. Please direct any questions to the organisers of your chosen workshop.

All the best,

Ulle Endriss and Francisco Melo
ECAI-2024 PC Chairs

\subsection{Workshop themes}

\begin{itemize}
\item AAAPEI: Adjustable Autonomy and and Physical Embodied Intelligence
\item ActSynt: Highlights of Reasoning about Actions, Planning and Reactive Synthesis
\item AIEB: Implementing AI Ethics through a Behavioural Lens
\item AIEER: International Workshop on AI in Education and Educational Research
\item AISUCMA: Workshop on Artificial Intelligence in Supply Chain Management
\item AREA: 4th Workshop on Agents and Robots for reliable Engineered Autonomy
\item ATT: 13th International Workshop on Agents in Traffic and Transportation
\item CLD2: Workshop on Classifier Learning From Difficult Data
\item CODAI: COuntering Disinformation with AI
\item CompAI: Workshop on Composite AI
\item CREAI: Workshop on Artificial Intelligence and Creativity
\item DAFUSAI: 2nd Workshop on Data Fusion for Artificial Intelligence
\item DAO-XAI: Data Meets Applied Ontologies in Explainable AI
\item EXPLIMED: Explainable Artificial Intelligence for the Medical Domain
\item FCA4AI: 12th Workshop on "What can FCA do for Artificial Intelligence?"
\item HAII5: Embracing Human-Aware AI in Industry 5.0
\item HYDRA: 3rd International Workshop on HYbrid Models for Coupling Deductive and Inductive ReAsoning
\item IMIS: Workshop on Intelligent Management Information Systems
\item LUHME: Language Understanding in the Human Machine Era
\item M-PREF: 15th Multidisciplinary Workshop on Advances in Preference Handling
\item MAI-XAI: Multimodal, Affective and Interactive eXplainable AI
\item ML-DE: Machine Learning Meets Differential Equations
\item PMAI: 3rd International Workshop on Process Management in the AI era
\item SC4AI: Social Choice for AI Ethics and Safety
\item VECOMP: International Workshop on AI Value Engineering and AI Compliance Mechanisms
\item WSCL: Workshop on Weakly Supervised and Cautious Learning: Bridging Machine Learning and Uncertainty Management
\item XRIA: First Workshop on "eXtended Reality \& Intelligent Agents"
\end{itemize}

